Large-scale Virtual Clinical Trials of Closed-loop Treatments for People with Type 1 Diabetes

We propose a virtual clinical trial for assessing the safety and efficacy of closed-loop diabetes treatments prior to an actual clinical trial. Such virtual trials enable rapid and risk-free pretrial testing of algorithms, and they can be used to compare different treatment variations for large and diverse populations. The participants are represented by multiple mathematical models, consisting of stochastic differential equations, and we use Monte Carlo closed-loop simulations to compute detailed statistics of the closed-loop treatments. We implement the virtual clinical trial using high-performance software and hardware, and we present an example trial with two mathematical models of one~million participants over 52~weeks (i.e., two~million simulations), which can be completed in 2~h 9~min.

==> tex/parameters.tex <==
\section{Parameters}
\begin{table*}
    \begin{center}
    \caption{Model parameters in the modified UVA/Padova model presented in Section~\ref{sec:models}.}
    \begin{tabular}{ c|c|c|c }
     \hline
     Symbol & Value or distribution & Unit & Description \\ 
     \hline
    \multicolumn{4}{c}{Model parameters in the model by~\citet{Hovorka:etal:2002, Hovorka:etal:2004} presented in Section~\ref{sec:models:hovorka}.} \\
     \hline
     $BW$       &  $U(65, 95)$                          & kg        & Body Mass   \\ 
     $EGP_0$    & $N(0.0161, 0.0039^2)$                 & mmol/min  & Liver glucose production at zero insulin  \\ 
     $F0_1$     & $N(0.0097, 0.0022^2)$                 & mmol/min  & Insulin independent glucose consumption \\
     $Ag$       & $U(0.7, 1.2)$                         & -         & CHO utilization  \\
     $k_{12}$   & $N(0.0649, 0.0282^2)$                 & 1/min     & Transfer Rate \\
     $k_{a1}$   & $N(0.0055, 0.0056^2)$                 & 1/min     & Deactivation Rate \\
     $k_{a2}$   & $N(0.0683, 0.0507^2)$                 & 1/min     & Deactivation Rate \\
     $k_{a3}$   & $N(0.0304, 0.0235^2)$                 & 1/min     &  Deactivation Rate \\
     $SIT$      & $N(51.2, 32.09^2)$                    & L/mU      & Transport insulin sensitivity \\
     $SID$      & $N(8.2, 7.84^2)$                      & L/mU      & Disposal insulin sensitivity \\
     $SIE$      & $N(520, 306.2^2)$                     & L/mU      & EGP insulin sensitivity \\
     $ke$       & $N(0.14, 0.035^2)$                    & 1/min     & Insulin elimination rate \\
     $V_I$      & $N(0.12, 0.012^2)$                    & L         & Insulin distribution volume   \\
     $V_G$      & $\ln(V_G) \sim N(\ln(0.15), 0.23^2)$   & L         & Glucose distribution volume \\
     $\tau_D$   & $\ln(1/\tau_D) \sim N(-3.689, 0.25^2)$ & min       & CHO absorption time constant\\ 
     $\tau_S$   & $1/\tau_S \sim N(0.018, 0.0045^2)$     & min       & Insulin absorption time constant \\
    \hline
    \multicolumn{4}{c}{Model parameters in the modified UVA/Padova model presented in Section~\ref{sec:models:uva:padova}.} \\
     \hline
    %  Symbol & Value or distribution & Unit & Description \\
    %  \hline
     $BW$ & $N(70.492, 12.7502^2)$          & kg                    & Body weight  \\
     $k_1$ & $N(0.0810, 0.0230^2)$      & 1/min                 & Diffusion constant of glucose subsystem  \\ 
     $k_2$ & $N(0.1370, 0.0530^2)$      & 1/min                 & Diffusion constant of glucose subsystem  \\ 
     $V_g$ & $N(1.8700, 0.1020^2)$        & dL/kg                 & Distribution volume of glucose subsystem \\
     $G_{b}$& $N(147.4100, 8.9390^2)$    & mg/kg                 & Basal plasma glucose  \\
     $HE_b$ & $0.6$        & -                 & Basal hepatic excretion \\
     $CL$ & $N(1.0210, 0.3080^2)$    & 1/min                 & Insulin clearance rate \\
     $m_1$ & $N(0.2109, 0.1362^2)$              & 1/min                 & Rate parameter of insulin subsystem \\
     $V_i$ & $N(0.0646, 0.0175^2)$       & L/kg                  & Distribution volume of insulin \\
     $I_b$ & $N(92.7470, 19.6618^2)$         & pmol/L                & Basal plasma insulin concentration \\
     $\tau_D$ & $\ln(1/\tau_D) \sim N(-3.689, 0.25^2) $     & min                   & Glucose apperance rate time constant \\
     $Ag$ & $U(0.7, 1.2)$           & -                     & CHO bioavailability \\
     $EGP_b$ & $N(2.5040, 0.3910^2)$      & mg/min                & Basal endogenous glucose production \\
     $k_{p2}$ & $N(0.0050, 0.0040^2)$     & 1/min                 & Liver glucose effectiveness \\
     $k_{p3}$ & $N(0.0106, 0.0068^2)$     & mg/kg/min per pmol/L  & Amplitude of insulin action on the liver \\
     $k_i$ & $N(0.0069, 0.0027^2)$      & 1/min                 & Delay between insulin signal and action rate parameter \\
     $F_{cns}$ & 1.0        & kg/kg/min             & Glucose uptake by the brain and erythrocytes \\
     $V_{mx}$ & $N(0.0810, 0.0330^2)$   & mg/kg/min per pmol/L  & Michaelis Menten equation parameter \\
     $K_{m0}$ & $N(224.2810, 12.2640^2)$     & mg/kg& Michaelis Menten equation parameter \\
     $p_{2U}$ & $N(0.0246, 0.012^2)$    & 1/min                 & Insulin action on the peripheral glucose utilization \\
     $k_{e1}$ & $0.0005 $     & 1/min                 & Glomerular filtration rate \\
     $k_{e2}$ & $339.0 $        & mg/kg                 & Renal threshold of glucose \\
     $k_{a1}$ & $N(0.0016, 0.0005^2)$      & 1/min                 & Subcutaneous insulin kinetics rate parameter \\
     $k_{a2}$ & $N(0.0149, 0.0052^2)$      & 1/min                 & Subcutaneous insulin kinetics rate parameter \\
     $k_{d}$ & $N(0.0161, 0.0017^2)$      & 1/min                 & Subcutaneous insulin kinetics rate parameter \\
     $k_{sc}$ & $N(0.1033, 0.0376^2)$      & 1/min                 & Diffusion constant of subcutaneous glucose subsystem \\
     \hline
    \end{tabular}
\end{center}
\end{table*}

% \begin{table*}
%     \begin{center}
%     \caption{Model parameters in the modified UVA/Padova model presented in Section~\ref{sec:models}.}
%     \begin{tabular}{ c|c|c|c } 
%      \hline
%      Symbol & Value or distribution & Unit & Description \\
%      \hline
%      $BW$ & $N(70.492, 12.7502^2)$          & kg                    & Body weight  \\
%      $k_1$ & $N(0.0810, 0.0230^2)$      & 1/min                 & Diffusion constant of glucose subsystem  \\ 
%      $k_2$ & $N(0.1370, 0.0530^2)$      & 1/min                 & Diffusion constant of glucose subsystem  \\ 
%      $V_g$ & $N(1.8700, 0.1020^2)$        & dL/kg                 & Distribution volume of glucose subsystem \\
%      $G_{b}$& $N(147.4100, 8.9390^2)$    & mg/kg                 & Basal plasma glucose  \\
%      $HE_b$ & $0.6$        & -                 & Basal hepatic excretion \\
%      $CL$ & $N(1.0210, 0.3080^2)$    & 1/min                 & Insulin clearance rate \\
%      $m_1$ & $N(0.2109, 0.1362^2)$              & 1/min                 & Rate parameter of insulin subsystem \\
%      $V_i$ & $N(0.0646, 0.0175^2)$       & L/kg                  & Distribution volume of insulin \\
%      $I_b$ & $N(92.7470, 19.6618^2)$         & pmol/L                & Basal plasma insulin concentration \\
%      $\tau_D$ & $\ln(1/\tau_D) \sim N(-3.689, 0.25^2) $     & min                   & Glucose apperance rate time constant \\
%      $Ag$ & $U(0.7, 1.2)$           & -                     & CHO bioavailability \\
%      $EGP_b$ & $N(2.5040, 0.3910^2)$      & mg/min                & Basal endogenous glucose production \\
%      $k_{p2}$ & $N(0.0050, 0.0040^2)$     & 1/min                 & Liver glucose effectiveness \\
%      $k_{p3}$ & $N(0.0106, 0.0068^2)$     & mg/kg/min per pmol/L  & Amplitude of insulin action on the liver \\
%      $k_i$ & $N(0.0069, 0.0027^2)$      & 1/min                 & Delay between insulin signal and action rate parameter \\
%      $F_{CNS}$ & 1.0        & kg/kg/min             & Glucose uptake by the brain and erythrocytes \\
%      $V_{mx}$ & $N(0.0810, 0.0330^2)$   & mg/kg/min per pmol/L  & Michaelis Menten equation parameter \\
%      $K_{m0}$ & $N(224.2810, 12.2640^2)$     & mg/kg& Michaelis Menten equation parameter \\
%      $p_{2U}$ & $N(0.0246, 0.012^2)$    & 1/min                 & Insulin action on the peripheral glucose utilization \\
%      $k_{e1}$ & $0.0005 $     & 1/min                 & Glomerular filtration rate \\
%      $k_{e2}$ & $339.0 $        & mg/kg                 & Renal threshold of glucose \\
%      $k_{a1}$ & $N(0.0016, 0.0005^2)$      & 1/min                 & Subcutaneous insulin kinetics rate parameter \\
%      $k_{a2}$ & $N(0.0149, 0.0052^2)$      & 1/min                 & Subcutaneous insulin kinetics rate parameter \\
%      $k_{d}$ & $N(0.0161, 0.0017^2)$      & 1/min                 & Subcutaneous insulin kinetics rate parameter \\
%      $k_{sc}$ & $N(0.1033, 0.0376^2)$      & 1/min                 & Diffusion constant of subcutaneous glucose subsystem \\
%      \hline
%     \end{tabular}
% \end{center}
% \end{table*}

% $F_{CNS}$ and $HE_b$ is set to 1 and 0.6 for both the healthy and T2D patient in Meal Simulation Model of the
% Glucose-Insulin System 2007. John has fixed ke1 and ke2 to the values of the healthy patient, i.e. $ke_1=0.0005$ and $ke_2=339$.
% \begin{table*}
%     \begin{center}
%     \caption{Model parameters in the model by~\citet{Hovorka:etal:2002, Hovorka:etal:2004} presented in Section~\ref{sec:models}.}
%     \begin{tabular}{ c|c|c|c } 
%      \hline
%      Symbol & Value or distribution & Unit & Description \\ 
%      \hline
%      $BW$       &  $U(65, 95)$                          & kg        & Body Mass   \\ 
%      $EGP_0$    & $N(0.0161, 0.0039^2)$                 & mmol/min  & Liver glucose production at zero insulin  \\ 
%      $F0_1$     & $N(0.0097, 0.0022^2)$                 & mmol/min  & Insulin independent glucose consumption \\
%      $Ag$       & $U(0.7, 1.2)$                         & -         & CHO utilization  \\
%      $k_{12}$   & $N(0.0649, 0.0282^2)$                 & 1/min     & Transfer Rate \\
%      $k_{a1}$   & $N(0.0055, 0.0056^2)$                 & 1/min     & Deactivation Rate \\
%      $k_{a2}$   & $N(0.0683, 0.0507^2)$                 & 1/min     & Deactivation Rate \\
%      $k_{a3}$   & $N(0.0304, 0.0235^2)$                 & 1/min     &  Deactivation Rate \\
%      $SIT$      & $N(51.2, 32.09^2)$                    & L/mU      & Transport insulin sensitivity \\
%      $SID$      & $N(8.2, 7.84^2)$                      & L/mU      & Disposal insulin sensitivity \\
%      $SIE$      & $N(520, 306.2^2)$                     & L/mU      & EGP insulin sensitivity \\
%      $ke$       & $N(0.14, 0.035^2)$                    & 1/min     & Insulin elimination rate \\
%      $V_I$      & $N(0.12, 0.012^2)$                    & L         & Insulin distribution volume   \\
%      $V_G$      & $\ln(V_g) \sim N(\ln(0.15), 0.23^2)$   & L         & Glucose distribution volume \\
%      $\tau_D$   & $\ln(1/\tau_D) \sim N(-3.689, 0.25^2)$ & min       & CHO absorption time constant\\ 
%      $\tau_S$   & $1/\tau_S \sim N(0.018, 0.0045^2)$     & min       & Insulin absorption time constant \\ 
%      \hline
%     \end{tabular}
% \end{center}
% \end{table*}

